Learning in Herding Mean Field Games: Single-Loop Algorithm with Finite-Time Convergence Analysis

We consider discrete-time stationary mean field games (MFG) with unknown dynamics and design algorithms for finding the equilibrium with finite-time complexity guarantees. Prior solutions to the problem assume either the contraction of a mean field optimality-consistency operator or strict weak monotonicity, which may be overly restrictive. In this work, we introduce a new class of solvable MFGs, named the "fully herding class", which expands the known solvable class of MFGs and for the first time includes problems with multiple equilibria. We propose a direct policy optimization method, Accelerated Single-loop Actor Critic Algorithm for Mean Field Games (ASAC-MFG), that provably finds a global equilibrium for MFGs within this class, under suitable access to a single trajectory of Markovian samples. Different from the prior methods, ASAC-MFG is single-loop and single-sample-path. We establish the finite-time and finite-sample convergence of ASAC-MFG to a mean field equilibrium via new techniques that we develop for multi-time-scale stochastic approximation. We support the theoretical results with illustrative numerical simulations. When the mean field does not affect the transition and reward, a MFG reduces to a Markov decision process (MDP) and ASAC-MFG becomes an actor-critic algorithm for finding the optimal policy in average-reward MDPs, with a sample complexity matching the state-of-the-art. Previous works derive the complexity assuming a contraction on the Bellman operator, which is invalid for average-reward MDPs. We match the rate while removing the untenable assumption through an improved Lyapunov function.

==> extra.tex <==
In discrete time, MFGs can be considered a generalization of MDPs and are widely solved using RL. Among the latest representative works, \citet{yang2018learning,carmona2021linear,perolat2021scaling} build upon policy optimization and \citet{anahtarci2020value,angiuli2022unified,angiuli2023convergence,gu2023dynamic,an2024does} consider valued-based methods. The algorithms proposed in these works, however, either do not come with convergence analysis or are only shown to converge asymptotically.

Finite-time convergent algorithms have been developed under the contraction assumption or strict weak monotonicity. Both assumptions imply the uniqueness of the mean field equilibrium, whereas multiple equilibria usually exist in practical applications.
Leveraging the contraction assumption or by enforcing the assumption through an entropy regularization, \citet{guo2019learning,xie2021learning,anahtarci2023q,mao2022mean,zaman2023oracle,yardim2023policy} design fixed-point-iteration-type algorithms, whose sample complexities we detail in Table 1.
\citet{perrin2020fictitious,geist2021concave,zhang2024learning} study solving strictly weakly monotone MFGs with mirror descent or fictitious play. 

In contrast, 
even when a MFG does not satisfy the herding condition with $\Delta=0$, there always exists a positive $\Delta$ for which the herding condition holds, and our algorithm is guaranteed to be stable in the sense that it roughly converges to a region around an equilibrium with radius $\sqrt{\Delta}$.

% It is worth pointing out the relevant works \citep{carmona2019linear,fu2020actor,zaman2020reinforcement,wang2024leader,koppel2024independent} on linear-quadrtic MFGs (i.e. the state and action are continuous, the cost is a quadratic function of state and action, and the state transition is linear), which can be regarded as an extension of the single-agent linear-quadratic regulator. The linear-quadratic structure makes this class of problems more convenient to study and efficient to solve.


% If the mean field has no impact on the transition kernel or reward function, the MFG reduces to a standard single-agent MDP, in which a simplified version of our proposed algorithm (that can be viewed as a variant of the actor-critic method) provably converges to a stationary point of the policy optimization objective. Finite-time analyses of (natural) actor-critic algorithms have been well-studied under discounted reward \citep{yang2018finite,barakat2022analysis,khodadadian2022finite} and average reward \citep{wu2020finite,panda2024critic,chen2024finite}.
% Improving over the state-of-the-art analysis in \citet{chen2024finite} for the average-reward setting, our algorithm enjoys a matching complexity without requiring an unrealistic assumption on the Bellman backup operator.

Let the parameter~$\theta\in\mathbb{R}^{|\Scal||\Acal|}$  encode the policy $\pi_{\theta}$. Consider iteratively refining the policy parameter $\theta$ along a direction that improves the cumulative reward under the induced mean field $\mu^{\star}(\pi_\theta)$. If we take $\theta'=\theta+\alpha\nabla_{\theta}J(\pi_{\theta},\mu)\mid_{\mu=\mu^{\star}(\pi_\theta)}$ with a sufficiently small step size $\alpha$, we can approximately guarantee
\begin{align*}
J(\pi_{\theta'},\mu^{\star}(\pi_\theta)) \gtrsim J(\pi_{\theta},\mu^{\star}(\pi_\theta)).
\end{align*}
However, the induced mean field shifts from $\mu^{\star}(\pi_\theta)$ to $\mu^{\star}(\pi_{\theta'})$ as the policy changes. Due to the lack of strong structure on $\mu^{\star}(\pi_{\theta})$ besides the Lipschitz condition, predicting/controlling whether $J(\pi_{\theta'},\mu^{\star}(\pi_{\theta'}))$ improves over $J(\pi_{\theta},\mu^{\star}(\pi_{\theta}))$ is difficult. 
In this work, we characterize the difficulty of an MFG by the mean field shift error $\Delta$ introduced in the following assumption.
A problem with a small or zero $\Delta$ is considered easier to solve. In fact, we later show in our analysis that the \texttt{ASAC-MFG} algorithm solves a MFG up to a sub-optimality gap proportional to $\Delta$.\looseness=-1
